An Introduction to the Summarization of Evolving Events: Linear and Non-linear Evolution

This paper examines the summarization of events that evolve through time. It discusses different types of evolution taking into account the time in which the incidents of an event are happening and the different sources reporting on the specific event. It proposes an approach for multi-document summarization which employs ``messages'' for representing the incidents of an event and cross-document relations that hold between messages according to certain conditions. The paper also outlines the current version of the summarization system we are implementing to realize this approach.

==> images/relations-example.latex <==
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(3062,1779)(91,-1018)
\thinlines
{\color[rgb]{0,0,0}\put(2071,209){\framebox(180,180){}}
}%
{\color[rgb]{0,0,0}\put(2071,-61){\framebox(180,180){}}
}%
{\color[rgb]{0,0,0}\put(2881, 29){\framebox(180,180){}}
}%
{\color[rgb]{0,0,0}\put(2881,-421){\framebox(180,180){}}
}%
{\color[rgb]{0,0,0}\put(2071,-691){\framebox(180,180){}}
}%
{\color[rgb]{0,0,0}\put(2161,299){\vector(-4, 3){  0}}
\put(2161,299){\vector( 4,-3){820.800}}
}%
\put(1981,-916){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Source 1}%
}}}}
\put(2701,-916){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Source 2}%
}}}}
\put(2206,-196){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}agreement}%
}}}}
{\color[rgb]{0,0,0}\put(361,164){\framebox(180,180){}}
}%
{\color[rgb]{0,0,0}\put(1261,164){\framebox(180,180){}}
}%
{\color[rgb]{0,0,0}\put(451,254){\vector(-1, 0){  0}}
\put(451,254){\vector( 1, 0){900}}
}%
\put(586,299){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}agreement}%
}}}}
{\color[rgb]{0,0,0}\put(361,-331){\framebox(180,180){}}
}%
{\color[rgb]{0,0,0}\put(1261,-331){\framebox(180,180){}}
}%
{\color[rgb]{0,0,0}\put(1621,749){\line( 0,-1){1755}}
}%
{\color[rgb]{0,0,0}\put(181,524){\vector( 0,-1){1305}}
}%
{\color[rgb]{0,0,0}\put(451,254){\vector( 0,-1){495}}
}%
{\color[rgb]{0,0,0}\multiput(2071,299)(-inf,-inf){1}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2070,297)(-inf,-inf){1}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2068,294)(-4.14710,-6.91183){2}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2064,287)(-5.00000,-10.00000){2}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2059,277)(-4.14705,-6.91175){3}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2051,263)(-4.50000,-9.00000){3}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2042,245)(-5.30000,-10.60000){3}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2031,224)(-3.86667,-7.73333){4}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2019,201)(-4.33333,-8.66667){4}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2006,175)(-4.66667,-9.33333){4}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1992,147)(-2.94828,-7.37069){5}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1979,118)(-3.03448,-7.58619){5}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1966, 88)(-3.12070,-7.80175){5}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1953, 57)(-2.77500,-8.32500){5}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1941, 24)(-2.75000,-8.25000){5}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1930, -9)(-2.90000,-8.70000){5}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1919,-44)(-2.30883,-9.23530){5}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1910,-81)(-1.90385,-9.51925){5}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1902,-119)(-1.32972,-7.97832){6}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1896,-159)(-1.35136,-8.10816){6}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\put(1892,-200){\line( 0,-1){ 41}}
\put(1891,-241){\line( 0,-1){ 40}}
\multiput(1892,-281)(1.52703,-9.16215){5}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1896,-318)(1.41892,-8.51355){5}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1902,-352)(2.50980,-10.03920){4}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1910,-382)(3.10000,-9.30000){4}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1919,-410)(3.93333,-7.86667){4}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1930,-434)(3.66667,-7.33333){4}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1941,-456)(4.14707,-6.91178){4}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1953,-477)(6.66000,-8.88000){3}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1966,-495)(6.42000,-8.56000){3}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1979,-512)(6.43900,-8.04875){3}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(1992,-528)(7.00000,-7.00000){3}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2006,-542)(6.50000,-6.50000){3}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2019,-555)(6.00000,-6.00000){3}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2031,-567)(11.40980,-9.50817){2}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2042,-577)(9.24590,-7.70492){2}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2051,-585)(8.00000,-6.00000){2}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\multiput(2059,-591)(12.48000,-9.36000){2}{\makebox(1.5875,11.1125){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
\put(2071,-600){\vector( 4,-3){0}}
}%
\put(451,569){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Linear/Synchrnous}%
}}}}
\put(1846,569){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Non-linear/Asynchronous}%
}}}}
\put( 91,-916){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}time}%
}}}}
\put(316,-691){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Source 1}%
}}}}
\put(1081,-691){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Source 2}%
}}}}
\put(496, 74){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}positive}%
}}}}
\put(496,-61){\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}graduation}%
}}}}
\put(1846,-556){\rotatebox{90.0}{\makebox(0,0)[lb]{\smash{{\SetFigFont{8}{9.6}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}termination}%
}}}}}
\end{picture}%


==> images/relations-linear.latex <==
\scriptsize\textbf{Performance}\\
  Assuming we have the following two messages:
  \begin{quote}
    performance (entity$_1$, in\_what$_1$, time\_span$_1$, value$_1$)\\
    performance (entity$_2$, in\_what$_2$, time\_span$_2$, value$_2$)
  \end{quote}
  Then the following Diachronic and Synchronic relations hold:
  \begin{quote}
    \textsl{Diachronic Relations}
      \begin{itemize}
        \item \textbf{Positive Graduation} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ < value$_2$)
        \item \textbf{Stability} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ = value$_2$)
        \item \textbf{Negative Graduation} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ > value$_2$)
      \end{itemize}
    \textsl{Synchronic Relations}
      \begin{itemize}
        \item \textbf{Agreement} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ = value$_2$)
        \item \textbf{Near Agreement} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ $\approx$ value$_2$)
        \item \textbf{Disagreement} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ $\neq$ value$_2$)
      \end{itemize}
  \end{quote}\normalsize

==> images/relations-nonlinear.latex <==
\scriptsize\textbf{Performance}\\
  Assuming we have the following two messages:
  \begin{quote}
    negotiate (entity$_{1a}$, entity$_{2a}$, about$_a$)\\
    negotiate (entity$_{1b}$, entity$_{1b}$, about$_b$)
  \end{quote}
  Then the following Diachronic and Synchronic relations hold:
  \begin{quote}
    \textsl{Diachronic Relations}
      \begin{itemize}
        \item \textbf{Positive Graduation} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ < value$_2$)
        \item \textbf{Stability} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ = value$_2$)
        \item \textbf{Negative Graduation} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ > value$_2$)
      \end{itemize}
    \textsl{Synchronic Relations}
      \begin{itemize}
        \item \textbf{Agreement} iff\\
              (entity$_{1a}$ = entity$_{1b}$) and (entity$_{2a}$ = entity$_{2b}$)\\
              and (about$_a$ = about$_b$)
        \item \textbf{Near Agreement} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ $\approx$ value$_2$)
        \item \textbf{Disagreement} iff\\
              (entity$_1$ = entity$_2$) and (in\_what$_1$ = in\_what$_2$) and\\
              (time\_span$_1$ = time\_span$_2$) and (value$_1$ $\neq$ value$_2$)
      \end{itemize}
  \end{quote}\normalsize

